The SDP value for random two-eigenvalue CSPs

We precisely determine the SDP value (equivalently, quantum value) of large random instances of certain kinds of constraint satisfaction problems, ``two-eigenvalue 2CSPs''. We show this SDP value coincides with the spectral relaxation value, possibly indicating a computational threshold. Our analysis extends the previously resolved cases of random regular $\mathsf{2XOR}$ and $\textsf{NAE-3SAT}$, and includes new cases such as random $\mathsf{Sort}_4$ (equivalently, $\mathsf{CHSH}$) and $\mathsf{Forrelation}$ CSPs. Our techniques include new generalizations of the nonbacktracking operator, the Ihara--Bass Formula, and the Friedman/Bordenave proof of Alon's Conjecture.

==> spectral-edge.tex <==
\subsection{Bounding the edges of the spectrum}
The proofs in this section follow the technical structure of proofs of Theorem 4.2 and Theorem 1.5 of \cite{AFH15}.

We use the notation $B_X$ to denote the nomadic walk matrix of $X$.
\begin{lemma}
    $\specrad\left(B_X\right) \le \frac{r_X}{2}$
\end{lemma}
\begin{proof}
    Recall that $\specrad(B_X) = \lim\limits_{k\to\infty} \|B_X^k\|_{2\to 2}^{1/k}$.  For each $k$, we give an upper bound on $\|B_X^k\|_{2\to 2}$.

    For directed edges $e,e'$ in $X$, if there is a \permissible~walk starting at $e$ and ending at $e'$ of the form $e = e_0,e_1,\dots,e_{k-1},e_k = e'$, it is unique.  We say $d(e,e') = k$ if there is such a nomadic walk, and $d(e,e') = \infty$ otherwise.  We use $\calP_{e,e'}$ to denote the sequence of $k+1$ edges $e_0,e_1,\dots,e_{k-1},e_k$.

    Then for any $f,g:\vec{E}(X)\to\R$, we have
    \begin{align*}
        \langle f, B_X^k g\rangle &= \sum_{(e,e'),d(e,e')=k} f(e)g(e') \prod_{i=1}^{k} (A_X)_i
    \end{align*}
    INCOMPLETE
\end{proof}

\begin{lemma}
    $\spec(X)\subseteq [\lambda_1+\lambda_2-r_X, \lambda_1+\lambda_2+r_X]$.
\end{lemma}
\begin{proof}
    INCOMPLETE
\end{proof}

==> triangle-ineq.tex <==
\subsection{Satisfying triangle inequalities}
Define $\widetilde{f}_v := \frac{f_v^{(1)}}{\|f_v^{(1)}\|}$.  A quantity of interest to us is $\langle \widetilde{f}_u, \widetilde{f}_v\rangle$ where $\{u,v\}$ is an edge.  Thus, we compute it below.
\begin{align*}
    \langle \widetilde{f}_u, \widetilde{f}_v\rangle &= \sum_{\alpha\in V(X)} \wt{f}_u(\alpha)\wt{f}_v(\alpha)\\
    &= \sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) < d(\alpha, v)}} \wt{f}_u(\alpha)\wt{f}_v(\alpha) + \sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) > d(\alpha, v)}} \wt{f}_u(\alpha)\wt{f}_v(\alpha) + \sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) = d(\alpha, v)}} \wt{f}_u(\alpha)\wt{f}_v(\alpha)\\
    &= \sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) < d(\alpha, v)}} \wt{f}_u(\alpha)^2\frac{A_{uv}(1-\delta)}{\sqrt{(c-1)(-\lambda_1\lambda_2)}} + \sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) > d(\alpha, v)}} \wt{f}_v(\alpha)^2\frac{A_{uv}(1-\delta)}{\sqrt{(c-1)(-\lambda_1\lambda_2)}} +\\ &\sum_{\substack{\alpha\in V(X)\\ d(\alpha, u) = d(\alpha, v)}} \sum_{w\in\Atom(u,v)} \wt{f}_w(\alpha)^2\frac{A_{uw}A_{wv}(1-\delta)^2}{\sqrt{(c-1)(-\lambda_1\lambda_2)}}
    \intertext{By switching the order of summations on the third term, applying \pref{fact:off-diag-square}, and then using identical ideas to the proof of \pref{lem:growth-rate} on all the terms, we can show to above is}
    &= \frac{2(c-1)}{c}\cdot\frac{A_{uv}(1-\delta)}{\sqrt{(c-1)(-\lambda_1\lambda_2)}} + \frac{(\lambda_1+\lambda_2)A_{uv}(1-\delta)^2}{(c-1)(-\lambda_1\lambda_2)}\cdot\frac{c-1}{c}\\
    &= \frac{A_{uv}(1-\delta)(r_X + (\lambda_1+\lambda_2)(1-\delta))}{c(-\lambda_1\lambda_2)}\\
    &= (1\pm\delta')A_{uv}\frac{r_X+(\lambda_1+\lambda_2)}{c(-\lambda_1\lambda_2)}
\end{align*}
INCOMPLETE SECTION
